Practical and Parallelizable Algorithms for Non-Monotone Submodular Maximization with Size Constraint

We present combinatorial and parallelizable algorithms for maximization of a submodular function, not necessarily monotone, with respect to a size constraint. We improve the best approximation factor achieved by an algorithm that has optimal adaptivity and nearly optimal query complexity to $0.193 - \varepsilon$. The conference version of this work mistakenly employed a subroutine that does not work for non-monotone, submodular functions. In this version, we propose a fixed and improved subroutine to add a set with high average marginal gain, ThreshSeq, which returns a solution in $O( \log(n) )$ adaptive rounds with high probability. Moreover, we provide two approximation algorithms. The first has approximation ratio $1/6 - \varepsilon$, adaptivity $O( \log (n) )$, and query complexity $O( n \log (k) )$, while the second has approximation ratio $0.193 - \varepsilon$, adaptivity $O( \log^2 (n) )$, and query complexity $O(n \log (k))$. Our algorithms are empirically validated to use a low number of adaptive rounds and total queries while obtaining solutions with high objective value in comparison with state-of-the-art approximation algorithms, including continuous algorithms that use the multilinear extension.

==> sec_ast_proof.tex <==
\section{The \adapst Algorithm}
% \begin{algorithm}[H]
%     \caption{The \adapst Algorithm}
%     \label{alg:atg}
%     \begin{algorithmic}[1]
%       \Procedure{AST}{$f, k, \epsi$}
%       \State \textbf{Input:} evaluation oracle $f:2^{\mathcal N} \to \reals$, constraint $k$,
%       accuracy parameter $\epsi > 0$
%       \State Initialize $M \gets \max_{x \in \mathcal N} f(x)$; 
%       $\ell \gets \lceil\log_{1 - \epsi}(1/(ck)))\rceil$; 
%       $c \gets 4 + \alpha$, where $\alpha^{-1}$ is ratio of \unc
%       \For{ $i \gets 0$ to $\ell$ in parallel}\label{line:forconcurrent}
%       \State $\tau_i \gets M \left( 1 - \epsi \right)^i$
%       \State $A_i,A_i' \gets \threseq \left( f, k, \tau_i, \epsi, 1 / 2 \right) $
%       \State $B_i,B_i' \gets \threseq \left( f\restriction_{\mathcal N\setminus A_i}, k, \tau_i, \epsi, 1 / 2 \right)$
%       \State $A_i'' \gets \unc (A_i)$
%       \State $C_i \gets \argmax \{ f(A_i'), f(B_i'), f(A_i'') \}$
%       \EndFor
%       \State \textbf{return} $C \gets \argmax_i \{ f(C_i) \}$
%       \EndProcedure
% \end{algorithmic}
% \end{algorithm}

\begin{theorem} 
    \label{thm:ast}
Suppose there exists an $(1/\alpha )$-approximation for
\unc with adaptivity $\Theta$ and query complexity
$\Xi$, and let $\epsi> 0$.
Then there exists an algorithm for \sm with
approximation ratio $\astRatio$ with probability
at least $1 - 1/n$, expected query complexity
$\oh{ \log_{1 - \epsi}(1/(ck))) \cdot \left( n / \epsi + \Xi \right) }$,
and adaptivity $\oh{\log( n) / \epsi + \Theta }$.  
\end{theorem}
\begin{proof}
    \textbf{Approximation Ratio.}
    \begin{lemma} \label{lemma:ast-guess}
        There exists $\tau_{i_0}$ that $\frac{(1-\epsi)\opt}{ck}\le \tau_{i_0}\le \frac{\opt}{ck}$.
    \end{lemma}
    \begin{proof}
        From submodularity, observe that 
        $$\tau_0=M\ge \sum_{o\in O}f(o)/k\ge f(O)/k > \frac{(1-\epsi)\opt}{ck}.$$
        Also,
        $$\tau_\ell=M(1-\epsi)^\ell\le M/ck \le \opt/ck.$$ 
        Since $\tau$ decreases with ratio $1-\epsi$ at each step, there exists a $\tau_{i_0}$ that
        $$\frac{(1-\epsi)\opt}{ck}\le \tau_{i_0}\le \frac{\opt}{ck}.$$
    \end{proof}
    
    Now let's consider the iteration with $\tau=\tau_{i_0}$.

    First,if the sets returned by \threseq follow that $|A_{i_0}|=k$ or $|B_{i_0}|=k$,
    w.l.o.g, let $|A_{i_0}|=k$.
    From Theorem~\ref{thm:threshold} and Lemma~\ref{lemma:ast-guess}, it holds that
    $$f(A_{i_0}')\ge(1-\epsi)\tau_{i_0}|A_{i_0}'|\ge \frac{(1-\epsi)^3\opt}{c}\ge (1/c-\epsi)\opt.$$
    Then,
    $$f(C)\ge f(A_{i_0}') \ge (1/c-\epsi)\opt.$$

    Second, if $|A_{i_0}|<k$ and $|B_{i_0}|<k$, from submodularity, 
    Theorem~\ref{thm:threshold} and Lemma~\ref{lemma:ast-guess},
    it holds that
    \begin{equation} \label{ineq:sub1}
        f(O\cup A_{i_0})-f(A_{i_0}) \le \sum_{o\in O\backslash A_{i_0}}\marge{o}{A_{i_0}} \le 
    \sum_{o\in O\backslash A_{i_0}} \tau_{i_0}\le \frac{\opt}{c},
    \end{equation}
    \begin{equation}\label{ineq:sub2}
        f((O\backslash A_{i_0})\cup B_{i_0})-f(B_{i_0})\le 
    \sum_{o\in (O\backslash A_{i_0})\backslash B_{i_0}}\marge{o}{B_{i_0}}\le 
    \sum_{o\in (O\backslash A_{i_0})\backslash B_{i_0}} \tau_{i_0}\le \frac{\opt}{c}.
    \end{equation}
    Then, we can bound the approximation ratio as follows,
    \begin{align*}
        \opt&=f(O)\le f(O \backslash A_{i_0})+ f(O\cap A_{i_0}) \numberthis \label{ineq:sub3}\\
        &\le f(O\cup A_{i_0}) + f((O\backslash A_{i_0})\cup B_{i_0})+ \alpha f(A_{i_0}'') \numberthis \label{ineq:sub4}\\
        &\le f(A_{i_0})+f(B_{i_0})+\frac{2\opt}{c}+\alpha f(A_{i_0}'') \numberthis \label{ineq:sub5}\\
        &\le f(A_{i_0}')+f(B_{i_0}')+\alpha f(A_{i_0}'')+\frac{2\opt}{c} \numberthis \label{ineq:sub6}\\
        &\le (2+\alpha)f(C_{i_0})+\frac{2\opt}{c},
    \end{align*}
    where Inequality~\ref{ineq:sub3} and~\ref{ineq:sub4} follow from submodularity, 
    Inequality~\ref{ineq:sub5} follows from Inequality~\ref{ineq:sub1} and~\ref{ineq:sub2},
    and Inequality~\ref{ineq:sub6} follows from Theorem~\ref{thm:threshold}.

    Therefore, $f(C)\ge f(C_{i_0})\ge \opt/c$.

    \textbf{Success Probability.}
    From Lemma~\ref{thm:threshold}, each call of \threseq succeeds with probability $1-\delta/2$.
    If the iteration with $\tau=\tau_{i_0}$ succeeds, Algorithm \adapst always succeeds.
    Then, the success probability of \adapst can be calculated as follows,
    $$\prob{\text{Algorithm~\ref{alg:ast} succeeds}} \ge 1-2\prob{\threseq \text{ fails}}\ge 1-\delta.$$

    % \textbf{Adaptivity and Query Complexity.}
    % The oracle queries occur within \threseq and \unc. 
    % And there are 2 \threseq and 1 \unc within an iteration.
    % Since the for loop is in parallel, the adaptivity is the linear combination
    % of $\oh{\log(n)/\epsi}$ and $\Theta$, which is $\oh{\log( n) / \epsi + \Theta }$.
    % And, the total queries are $\oh{ \log_{1 - \epsi}(1/(6k)) \cdot \left( n / \epsi + \Xi \right) }$.
\end{proof}

==> sec_atg_proof.tex <==
\section{The \adaptg Algorithm}
 
 \begin{theorem} \label{thm:atg}
    Suppose there exists an $(1/\alpha)$-approximation for
    \unc with adaptivity $\Theta$ and query complexity
    $\Xi$, and let $\epsi> 0$.
    Then the algorithm \adaptg  for \sm
    has approximation ratio
    $\atgRatio$ with probability at
    least $1 - 1/n$,
    adaptive complexity of
    $O\left( \log( n ) / \epsi + \Theta \right)$ 
    and expected query complexity of
    $O \left( \log_{1 - \epsi}(1/(6k)) \cdot \left( n / \epsi \right) + \Xi \right)$.
\end{theorem}
\begin{proof}
  Let $(a_j)$ be a sequence with $k$ elements, 
  while the first $|A|$ elements are $A$,
  and the rest are $a_0$s, where 
  $a_0$ is defined as element with 0 marginal gain which means $\marge{a_0}{S}=0$
  for any $S \subseteq \mathcal{N}$.
  And let $(a_j')$ be a subsequence of $(a_j)$, where $a_j'$ has nonnegative marginal gain.
  Then, $(a_j')$ is the sequence of $A'$.

  Let $\mathcal{A}_j'=\{a_1',\cdots,a_j'\}$, 
  $A_i$ be the set $A$ returned at the end of iteration $i$,
  $A_{-1}=\emptyset$,
  $a_j'$ be returned at iteration $i(j)$.
  If $a_j'=a_0$, let $i(j)=\ell+1$.
  Define $\mathcal{B}_j'$ and $B_{i(j)}$ analogously.

  \textbf{Approximation Ratio.}
  \begin{lemma} \label{lemma:seq1}
    There are at least $\lceil(1-\epsi')k\rceil$ of $j$ that 
    $$f(\mathcal{A}_j')-f(\mathcal{A}_{j-1}')+\frac{M}{ck}\ge 
    \frac{1-\epsi'}{k}\left(f(O\cup A_{i(j)-1})-f(\mathcal{A}_{j-1}')\right).$$
    And for any $j$,
    $$f(\mathcal{A}_j')\ge f(\mathcal{A}_{j-1}').$$
  \end{lemma}
  \begin{proof}
    Since $a_j'$ has nonnegative marginal gain, it always holds that 
    $f(\mathcal{A}_j')\ge f(\mathcal{A}_{j-1}')$.

    From Lemma~\ref{lemma:ThresholdGood}, there are at least $(1-\epsi)$-fraction
    of $A$ are good elements.
    Therefore, there are at least $(1-\epsi)k$ of $a_j'$ which is good 
    or $a_j'=a_0$.
    Next, let's consider the following 3 cases of those $a_j'$s.

    \textbf{Case} $i(j)=0$ and $a_j'$ is good.
    By Theorem~\ref{thm:threshold} and Lemma~\ref{lemma:ThresholdGood}, it holds that 
    $$f(\mathcal{A}_j')-f(\mathcal{A}_{j-1}')\ge \tau_0=M \ge \frac{1}{k} \sum_{o \in O}f(o)\ge \frac{1}{k}f(O).$$

    \textbf{Case} $i(j)>0$ and $a_j'$ is good.
    Since $a_j'$ is returned at iteration $i(j)$ and $a_j'$ is good, it holds that:
    (1) $f(\mathcal{A}_j')-f(\mathcal{A}_{j-1}')\ge \tau_{i(j)}$; 
    (2) at previous iteration $i(j)-1$, \threseq returns $S_{i(j)-1}$ that $|S_{i(j)-1}| < k-|A_{i(j)-2}|$.
    From property (2) and Theorem~\ref{thm:threshold}, for any $o \in O\backslash A_{i(j)-1}$,
    $\marge{o}{A_{i(j)-1}} < \tau_{i(j)-1}$.
    Then,
    \begin{align*}
      f(\mathcal{A}_j')-f(\mathcal{A}_{j-1}')&\ge \tau_{i(j)}= (1-\epsi')\tau_{i(j)-1}\\
      &> \frac{1-\epsi'}{k}\sum_{o\in O\backslash A_{i(j)-1}}\marge{o}{A_{i(j)-1}}\\
      &\ge \frac{1-\epsi'}{k}\left(f(O\cup A_{i(j)-1})-f(A_{i(j)-1})\right)\\
      &\ge \frac{1-\epsi'}{k}\left(f(O\cup A_{i(j)-1})-f(A'_{i(j)-1})\right) \numberthis \label{ineq:sub8}\\
      &\ge \frac{1-\epsi'}{k}\left(f(O\cup A_{i(j)-1})-f(\mathcal{A}_{j-1}')\right), \numberthis \label{ineq:sub7}
    \end{align*}
    where Inequality~\ref{ineq:sub8} follows from the proof of Lemma~\ref{lemma:ThresholdGood},
    and Inequality~\ref{ineq:sub7} follows from $A'_{i(j)-1} \subseteq \mathcal{A}_{j-1}'$.

    \textbf{Case} $i(j)=\ell+1$ (or $a_j'=a_0$). In this case, $i(j)-1=\ell$ and $|A|<k$ when the \textbf{for} loop ends.
    So, \threseq in the last iteration returns $S_\ell$ that $|S_\ell| < k-|A_{\ell-1}|$.
    From Theorem~\ref{thm:threshold}, it holds that $\marge{o}{A_{\ell}} < \tau_\ell < \frac{M}{ck}$, 
    for any $o \in O\backslash A_{\ell}$.
    Thus,
    $$\frac{M}{ck}> \frac{1}{k}\sum_{o\in O\backslash A_{\ell}} \marge{o}{A_{\ell}}\ge 
    \frac{1}{k}\left(f(O\cup A_\ell) - f(A_\ell)\right).$$

    The first inequality of Lemma~\ref{lemma:seq1} holds in those three cases
    with at least $(1-\epsi')k$ of $j$.
  \end{proof}

  Following the notation and proof of Lemma~\ref{lemma:seq1},
  we can get a similar lemma for set $B$.
  \begin{lemma} \label{lemma:seq2}
    There are at least $\lceil(1-\epsi')k\rceil$ of $j$ that 
    $$f(\mathcal{B}_j')-f(\mathcal{B}_{j-1}')+\frac{M}{ck}\ge 
    \frac{1-\epsi'}{k}\left(f((O\backslash A)\cup B_{i(j)-1})-f(\mathcal{B}_{j-1}')\right).$$
    And for any $j$,
    $$f(\mathcal{B}_j')\ge f(\mathcal{B}_{j-1}').$$
  \end{lemma}

  \begin{lemma} \label{lemma:seq3}
    Let $\Gamma_u=f(\mathcal{A}_{j(u)}')+f(\mathcal{B}_{j(u)}')$, 
    where $a_{j(u)}'$ is the $u$-th
    good element or $a_0$, the same as $b_{j(u)}'$.
    Then, there are at least $\lceil(1-\epsi')k\rceil$ of $u$ follow that
    $$f(O\backslash A)-\Gamma_u-\frac{2M}{c(1-\epsi')}\le 
    \left(1-\frac{1-\epsi'}{k}\right)\left(f(O\backslash A)-\Gamma_{u-1}-\frac{2M}{c(1-\epsi')}\right).$$
  \end{lemma}
  \begin{proof}
    From Lemma~\ref{lemma:seq1}, $f(\mathcal{A}_{j(u)-1})\ge f(\mathcal{A}_{j(u-1)})$, and
    \begin{align*}
      f(\mathcal{A}_{j(u)}')& \ge \left(1-\frac{1-\epsi'}{k}\right)f(\mathcal{A}_{j(u)-1}')+
      \frac{1-\epsi'}{k}f(O\cup A_{i(j(u))-1})-\frac{M}{ck}\\
      &\ge \left(1-\frac{1-\epsi'}{k}\right)f(\mathcal{A}_{j(u-1)}')+
      \frac{1-\epsi'}{k}f(O\cup A_{i(j(u))-1})-\frac{M}{ck}.
    \end{align*}
    Similarly,
    $$f(\mathcal{B}_{j(u)}')\ge \left(1-\frac{1-\epsi'}{k}\right)f(\mathcal{B}_{j(u-1)}')+
    \frac{1-\epsi'}{k}f((O\backslash A)\cup B_{i(j(u))-1})-\frac{M}{ck}.$$
    From the above two inequality and submodularity,
    \begin{align*}
      \Gamma_u&\ge \left(1-\frac{1-\epsi'}{k}\right) \Gamma_{u-1}+
      \frac{1-\epsi'}{k}\left(f(O\cup A_{i(j(u))-1})+f((O\backslash A)\cup B_{i(j(u))-1})\right)-\frac{2M}{ck}\\
      &\ge \left(1-\frac{1-\epsi'}{k}\right) \Gamma_{u-1}+\frac{1-\epsi'}{k} f(O\backslash A)-\frac{2M}{ck}.
    \end{align*}
  \end{proof}

  From Lemma~\ref{lemma:seq3},
  \begin{align*}
    &f(O \backslash A)-f(A')-f(B')-\frac{2M}{c(1-\epsi')} \\
    &\le f(O \backslash A)-\Gamma_{\lceil(1-\epsi')k\rceil}-\frac{2M}{c(1-\epsi')}\\
    &\le \left(1-\frac{1-\epsi'}{k}\right)^{(1-\epsi')k}\left(f(O\backslash A)-\frac{2M}{c(1-\epsi')}\right)\\
    &\le e^{-(1-\epsi')^2}\left(f(O\backslash A)-\frac{2M}{c(1-\epsi')}\right).
  \end{align*}
  Let $\beta=1-e^{-(1-\epsi')^2}$,
  \begin{align*}
    f(O\backslash A)&\le \frac{1}{\beta}\left(f(A')+f(B')\right)+\frac{2M}{c(1-\epsi')}\\
    &\le \frac{1}{\beta}\left(f(A')+f(B')\right)+\frac{2f(O)}{c(1-\epsi')}.
  \end{align*}

  Since an $(1/\alpha)$-approximation is used for \unc on $A$,
  $f(O\cap A) \le \alpha f(A'').$

  From submodularity and the above results,
  \begin{align*}
    f(O)&\le f(O\cap A) + f(O\backslash A)\\
    &\le \alpha f(A'')+\frac{1}{\beta}\left(f(A')+f(B')\right)+\frac{2f(O)}{c(1-\epsi')}\\
    &\le \left(\alpha+\frac{2}{\beta}\right)f(C) + \frac{2f(O)}{c(1-\epsi')}.
  \end{align*}
  Therefore,
  \begin{align*}
    f(C)&\ge \frac{1-\frac{2}{c(1-\epsi')}}{\alpha+\frac{2}{\beta}}f(O)\\
    &\ge \left(\frac{e-1}{\alpha(e-1)+2e}-\epsi\right)f(O).
  \end{align*}

  \textbf{Success Probability.}
  For a single \threseq, the failure probability is less than $\delta'$.
  \adaptg has $2\ell$ calls of \threseq.
  Therefore, the success probability of \adaptg can be bounded as follows,
  $$\prob{\text{ATG succeeds}}\ge 1-2\ell\cdot \prob{\threseq \text{ fails}}\ge 
  1-2\ell \cdot \frac{\delta}{2\ell}=1-\delta.$$

\end{proof}
  
